ACS: Concurrent Kernel Execution on Irregular, Input-Dependent Computational Graphs

GPUs are widely used to accelerate many important classes of workloads today. However, we observe that several important emerging classes of workloads, including simulation engines for deep reinforcement learning and dynamic neural networks, are unable to fully utilize the massive parallelism that GPUs offer. These applications tend to have kernels that are small in size, i.e., have few thread blocks that do not saturate compute resources. Executing independent kernels concurrently is a promising approach to improve parallelism and utilization. However, this inter-kernel concurrency is difficult to leverage in such workloads with existing approaches: First, the inter-kernel dependencies and computational graph are input-dependent and vary each time the application is executed. Second, the computational graphs tend to be irregular, requiring fine-grain scheduling and synchronization; thus incurring significant synchronization overheads if kernel execution is parallelized. In this work, we propose ACS, a framework that enables lightweight detection of inter-kernel dependencies and low overhead kernel scheduling at runtime. The key idea behind ACS is to perform inter-kernel dependency checks for a small window of kernels at runtime, similar to out-of order instruction scheduling. This enables concurrent execution of kernels in applications whose computational graphs are input dependent and require fine-grained scheduling. We propose ACS-SW, a software-only open-source implementation of ACS and ACS-HW, a hardware-software cooperative implementation. ACS-HW further reduces synchronization overheads by reducing communication between the CPU and GPU. We evaluate ACS for deep RL simulation and dynamic DNNs on both real hardware and a GPU simulator. We demonstrate speedups of up to 2.19x (1.56x on average) by improving GPU utilization with concurrent kernel execution.

==> textsrcs/background.tex <==

% % \subsection{GPU Programming Model}
% % \outlinepoint{GPU Architecture Model outline:
% % \begin{itemize}
% %     \item GPU kernels are divided into thread blocks, and the number of active blocks that at runtime.
% %     \item Describe what occupancy is, and the resources used/occupied by GPU kernel at launch time,
% %     \item Modern GPUs (V100) could have up to active resident simultaneously blocks at runtime.
% % \end{itemize} 
% % }

% % GPU programs comprise \emph{kernels} that are parallel sections of the code executed on the GPU.
% % GPU kernels are in turn composed of a 3-dimensional set of cooperative thread arrays (CTAs) or thread blocks. Each thread block is further composed of a 3D array of threads. This hierarchy of threads in a kernel enables parallelizing across the streaming multiprocessors (SMs) of the GPU, which execute threads using SIMD execution.

% %Each thread block is assigned to a single SM, and once scheduled for execution, becomes an "active".
% %The GPU consists of a number of SMs, and each SM can fetch instructions from multiple thread blocks at a time.
% % Modern GPUs are capable of running at having over 500 active resident thread blocks simultaneously, known as a wavefront. 
% % A GPU kernel which has thread blocks over this limit divides them into multiple wavefronts.


% % \vspace{-0.2cm}
% \subsection{GPU Architecture}
% % \vspace{-0.2cm}
% \begin{outlineenv}

% %A high level diagram of a GPU architecture is shown in Figure~\ref{fig:gpu_base}, representative of modern GPU architectures.

% \outlinepoint{GPU Architecture Model outline:
% \begin{itemize}
%     \item GPU kernels are divided into thread blocks, and the number of active blocks that at runtime.
% \end{itemize}
% }

% % A GPU consists of multiple SIMT cores, or streaming multiprocessors (SMs), a kernel management unit (KMU) which maintains multiple hardware queues (or \emph{streams}) which schedules kernels launch. 
% The device runtime executing on the CPU issues commands (kernel launch, memory operations, etc.) to the GPU at every flush interval over PCIe. 
% When a kernel is launched, the CPU passes kernel arguments, kernel dimensions, and other metadata (like the stream, shared memory resources, etc.) to the GPU. The Kernel Management Unit (KMU), tracks and schedules kernels for execution to the kernel dispatch unit (KDU). Thread blocks from the kernels in the KDU are then scheduled for execution at the streaming multiprocessors (SMs). Each SM can concurrently execute a fixed number of thread blocks (determined by the resources required by the thread block) using fine-grained multithreading.  
% The launched kernels are tracked by a kernel dispatch unit, whose blocks are forwarded to the SMs by a thread block scheduler.
% % These commands are either kernel launches, device memory operations, synchronization events, etc.
% % The IO unit on the GPU forwards kernel launches to a kernel management unit (KMU). 


% \begin{figure}[!htb]
%     % \vspace{-0.2cm}
%     \centering
%     \includegraphics[width=.55\linewidth]{figs/gpubase.pdf}
%     % \vspace{-0.1cm}
%     \caption{Kernel scheduling and dispatch on a GPU.}
%     \label{fig:gpu_base}
%     % \vspace{-0.4cm}
% \end{figure}



% \outlinepoint{GPU SM Resources and Occupancy
% \begin{itemize}
%     \item GPU kernels are divided into thread blocks, and the number of active blocks that at runtime.
%     \item Describe what occupancy is, and the resources used/occupied by GPU kernel at launch time,
%     \item Modern GPUs (V100) could have up to active resident simultaneously blocks at runtime.
% \end{itemize}
% }


% \outlinepoint{
% \begin{itemize}
%     \item Increasing number of device SMs and underutilization, 
%     \item different configuration, 
%     \item Warp scheduler
% \end{itemize}}

% \end{outlineenv}

% % \subsection{GPU Stream Abstraction}
% GPU stream~\cite{cudastream} is a sequence of GPU commands issued by the CPU which execute in issue-order on the GPU. 
% These GPU commands can be kernel launches, memory copy operations, memory set operations, etc.
% Modern GPUs provide support for multiple streams, where a host (CPU) can issue GPU operations concurrently.
% This enables running multiple kernels on the GPU to increase performance.
% A GPU stream operation can be executed in an asynchronous way, where the CPU continues executing code while the GPU operation waits to be executed by the GPU. For the host to use data produced by the GPU kernels, the host must explicitly synchronize and wait until the kernel has completed execution.


% % \begin{itemize}
% %     \item GPU streams allow execution of kernels in the same order in which they are queued up in the stream.
% %     \item Launching kernels on separate streams requires explicit synchronization to be done, which 
% %     \item Streams correspond to hardware queues in the device in the kernel management unit(KMU)
% % \end{itemize}

% % GPU streams allow execution of kernels in the same order in which they are queued up in the stream.



% % \subsection{Underutilization of GPU resources}
% % GPU underutilization occurs when compute units in the GPU remain idle during kernel execution. 
% % Underutilization can be the result of a number of factors. 
% % Reasons for GPU underutilization:
% % \begin{itemize}
% %     \item small grid launches with single kernel
% %     \item kernel launch overhead resulting in idle GPU time, 
% %     \item tail effect,
% %     \item scheduling and issue overhead
% %     \item Pipeline stalls in the algorithm
% % \end{itemize}

% % Small grid launches:
% % A modern V100 GPU has 80 SMs, each capable of running $6$ active resident blocks per SM is capable of running $800$ active resident blocks executing simultaneously. 
% % GPU kernel launches with batch size: 




% % \subsection{Scheduling overhead}
% % \begin{outlineenv}


% % \outlinepoint{a majority of DL workloads use regular tensor computation to leverage GPU parallelism. However, architectures }

% % \outlinepoint{A number of deep learning frameworks differentiate between are designed to schedule at runtime. As a result, a number of these frameworks opportunistically.}

% % \outlinepoint{large number of steps to be performed. The sequence of operators to be launched to execute the static graph are known apriori.}

% % \outlinepoint{third party frameworks like Cudnn, mkldnn, etc. have a number of operators to perform. These implementations contain a choice of a large number of operations for corresponding hardware for different data types and shapes which}

% % \outlinepoint{Several recent approaches attempt to reduce the schedule time overhead with many techniques~\cite{}}

% % \end{outlineenv}




\subsection{Background and Prior Mechanisms}
\label{sec:approach_prior_mechanisms}
\insertionhpca{Figure~\ref{fig:gpuwq} shows an overview of the hardware model in modern GPU architectures~\cite{oversubscribed_queues}. The host communicates with the command processor (CP) of the GPU via a virtual memory region which is memory mapped to the GPU, accessible by the command processor. This enables communication between the CPU and GPU through entries in the command queue. The CPU transmits kernel launch packets to the GPU by writing them to the user mode command queue.  
The CP is responsible for decoding and dispatching the kernels in these command queues for execution. The CP accesses the command queue and schedules the kernels at the head for execution. This ensures that the kernels are dispatched for launch from these queues in order.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.7\linewidth]{figs/gpuwq.png}
    % %\vspace{-0.2cm}
\caption{Scheduling kernels from multiple streams}
\label{fig:gpuwq}
%%\vspace{-0.1cm}
\end{figure}


The GPU runtime can launch kernels into different streams. These streams are mapped to one of the command queues in the device-mapped memory of the GPU. The command processor schedules kernels at the head of these queues concurrently, thus enabling concurrent kernel execution. 
However, neither the CP nor the kernel launch packets in the command queues have information on inter-kernel data dependencies. Kernels in different queues are assumed to be independent of each other and all kernels within the same queue are executed in order. Hence, in order to leverage parallelism in kernel executions, the task of checking inter-kernel dependencies and determining the kernels which can execute concurrently (and thus scheduling into different queues) \emph{has to be done by the host application.} However, this is a problem, as this adds significant dependency-checking/scheduling latency to the run time. It also requires communication with the host (through a synchronization routine) to be performed each time a kernel completes execution, adding to the overhead.  



==> textsrcs/implementation_notes.tex <==
\hpcarebuttal{
\textbf{Performance implication in general workloads}: Our HW mechanism is intended for workloads that launch several short-running kernels, which do not fully utilize the GPU. 
A trivial approach to doing this is to use a higher batch size. A higher batch size would result in higher execution time for each kernel, leading to the time required for synchronization being a much lower percentage of the overall runtime. In these cases, we would observe the same performance on using ACE as the baseline.
Hence, using ACE on workloads that have a high GPU utilization or in workloads with long-running kernels compared to the synchronization times results in performance equivalent to the baseline implementation. However, the primary focus of this work is to demonstrate the lower latency needed for executing these workloads, and increasing the batch size is not sufficient to achieve this.
}

\hpcarebuttal{
\textbf{SRAM-free implementation in \Xlabel{}-HW}: \Xlabel{}-HW currently requires the use of an SRAM module in the command processor of the GPU. In order to implement an SRAM-free design, an equivalent architecture to \Xlabel{}-HW can be envisioned in which an embedded processor does the kernel dispatch to the GPU. This design would remove the requirement of SRAM modules for \Xlabel{}-HW. The embedded processor and the GPU command processor signal information on kernel completions and new kernel dispatches. The communication between the embedded processor and the GPU proceeds via a mapped global memory region of the GPU to the embedded processor’s virtual memory. The additional overhead in this mechanism compared to \Xlabel{}-HW is the result of this communication latency as well as the additional driver software execution latency of the embedded processor.
}

